Towards Non-Volatile Spin Orbit Devices: Deposition of Ferroelectric Hafnia on Monolayer Graphene/Co/HM Stacks

Although technologically challenging, the integration of ferroelectric thin films with graphene spintronics potentially allows the realization of highly efficient, electrically tuneable, non-volatile memories. Here, the atomic layer deposition (ALD) of ferroelectric Hf$_{0.5}$Zr$_{0.5}$O$_2$ (HZO) directly on graphene (Gr)/Co/heavy metal (HM) epitaxial stacks is investigated via the implementation of several nucleation methods. With an in-situ method employing an Al$_2$O$_3$ layer, the HZO demonstrates a remanent polarization (2Pr) of 19.2 $\mu C/cm^2$. An ex-situ, naturally oxidized sputtered Ta layer for nucleation produces a film with 2Pr of 10.81 $\mu C/cm^2$, but a lower coercive field over the stack and switching enduring over subsequent cycles. Magnetic hysteresis measurements taken before and after ALD deposition show strong perpendicular magnetic anisotropy (PMA), with only slight deviations in the magnetic coercive fields due to the HZO deposition process, thus pointing to a good preservation of the single-layer Gr. X-ray diffraction measurements further confirm that the high-quality interfaces demonstrated in the stack remain unperturbed by the ferroelectric deposition and anneal.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

